Driver Surge Pricing

Ride-hailing marketplaces like Uber and Lyft use dynamic pricing, often called surge, to balance the supply of available drivers with the demand for rides. We study driver-side payment mechanisms for such marketplaces, presenting the theoretical foundation that has informed the design of Uber's new additive driver surge mechanism. We present a dynamic stochastic model to capture the impact of surge pricing on driver earnings and their strategies to maximize such earnings. In this setting, some time periods (surge) are more valuable than others (non-surge), and so trips of different time lengths vary in the induced driver opportunity cost. First, we show that multiplicative surge, historically the standard on ride-hailing platforms, is not incentive compatible in a dynamic setting. We then propose a structured, incentive-compatible pricing mechanism. This closed-form mechanism has a simple form and is well-approximated by Uber's new additive surge mechanism. Finally, through both numerical analysis and real data from a ride-hailing marketplace, we show that additive surge is more incentive compatible in practice than is multiplicative surge.

==> app_simulations.tex <==
\section{Simulations}



Here, we show how the additive and multiplicative surge compare in terms of approximate incentive compatibility as a function of the model primitives. In Figure~\ref{fig:affineapprox} in the main text, we show how the fraction of accepted trips changes with some primitives. Here, we show the same plots but as other model primitives change, and with other parameter sets. 


\begin{figure}[H]
	\centering
\begin{subfigure}[t]{0.48\textwidth}
	\centering
	\includegraphics[width=\linewidth]{plots/percrejected/Fraction_accepted_changewithlam21.pdf}	
	\caption{With $\lonetwo$, rate of surge starting.}
\end{subfigure}
~ \hfill	\begin{subfigure}[t]{0.48\textwidth}
	\centering
	\includegraphics[width=\linewidth]{plots/percrejected/Fraction_accepted_changewithlam1.pdf}	
	\caption{With $\lambda_1$, arrival rate of jobs in state $1$.}
\end{subfigure}~\hfill

	\caption{How the fraction of trips accepted varies primitives, fixing reward in the non-surge state $R_1 = 1$. When not varied, the primitives are $\lambda_1 = \lambda_2 = 20, \lonetwo = 1, \ltwoone = 4, R_2 = 3$, and the mean trip length is $\frac{1}{3}$. }
	\label{fig:affineapprox_otherprimitives}
\end{figure}


\begin{figure}[H]
	\centering
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{plots/pricing/Fraction_accepted_changewithR1ratio.pdf}	
		\caption{With $R_2$.}
		\label{fig:fracacceptedchangewithR1_pricing}
	\end{subfigure}
	~ \hfill
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{plots/pricing/Fraction_accepted_changewithmtl.pdf}	
		\caption{With mean trip length, i.e. mean of $F_1,F_2$.}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{plots/pricing/Fraction_accepted_changewithlam2.pdf}	
		\caption{With $\lambda_2$, arrival rate of jobs in state $2$.}
	\end{subfigure}
	~ \hfill
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{plots/pricing/Fraction_accepted_changewithlam21.pdf}	
		\caption{With $\lambda_{21}$, rate of surge ending.}
	\end{subfigure}
\end{figure}

\begin{figure}[H]
	\centering
	\ContinuedFloat
	
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{plots/pricing/Fraction_accepted_changewithlam1.pdf}	
		\caption{With $\lambda_1$, arrival rate of jobs in state $1$.}
	\end{subfigure}
	~ \hfill
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=\linewidth]{plots/pricing/Fraction_accepted_changewithlam12.pdf}	
		\caption{With $\lambda_{12}$, rate of surge starting.}
	\end{subfigure}
	~ \hfill
	\caption{How the fraction of trips accepted varies with the reward in the surge state and the mean trip length, fixing reward in the non-surge state $R_1 = 1$. When not varied, the primitives are $\lambda_1 = \lambda_2 = 12, \lonetwo = 1, \ltwoone = 4, R_2 = \frac{3}{2}$, and the mean trip length is $\frac{1}{3}$. Other primitive values and variations are shown in the Appendix. }
	\label{fig:affineapprox_pricingprimitives}
\end{figure}

==> related_short.tex <==
\subsection{Related Work}
We discussed some of the related work on surge pricing above. Here, we briefly review the lines of research closest to ours, setting aside, e.g., other works in pricing and matching~\citep{ozkan_dynamic_2016,banerjee2017pricing,banerjee_segmenting_2017,feng2017we,zhang2017taxi,banerjee_state_2018,hu2018dynamic,korolko_dynamic_2018,ozkan2018joint,ashlagi2018maximizing,kanoria_near_2019}. We refer the reader to a recent survey by~\citet{korolko_dynamic_2018} for a broader overview of the growing literature on ride-hailing markets.

\textbf{Driver spatio-temporal strategic behavior.} Several works model strategic driver behavior in a spatial network structure, and across time in a single-state. \citet{ma_spatio-temporal_2018} develop spatially and temporally smooth prices that are welfare-optimal and incentive compatible in a deterministic model. %
We similarly seek to develop incentive compatible pricing schemes, and both works broadly construct VCG-like prices that account for driver opportunity costs. Our focus is on structural aspects (e.g. multiplicative in trip length) in a non-deterministic model.
\citet{bimpikis_spatial_2016} show how the platform would price trips between locations, taking into account strategic driver re-location decisions, in a single-state model with discrete locations. They show that pricing trips based on the origin location substantially improves surplus, as well as the benefits of ``balanced'' demand patterns.
 \citet{besbes_surge_2018} consider a continuous state space setting and show how a platform may optimally set prices across the space in reaction to a localized demand shock to encourage drivers to relocate. They find that localized prices have a global impact, and, e.g., the optimal pricing solution incentivizes some drivers to move away from a demand shock. ~\citet{afeche_ride-hailing_2018},~\citet{guda_your_2019}, and~\citet{yang2018mean} also deliver important insights.










\textbf{{Dynamic pricing in ride-hailing and service systems}.}
There is a growing literature on queuing and service systems motivated in part by ride-hailing markets.
For example, \citet{besbes_spatial_2018} revisit the classic square root safety staffing rule in spatial settings, cf.,~\cite{bertsimas_stochastic_1991,bertsimas_stochastic_1993}.
Much of the focus of this line of work is how pricing affects the arrival rate of (potentially heterogeneous) customers, and thus the trade-off between the price and rate of customers served in maximizing revenue.

\citet{banerjee_pricing_2015} consider a network of queues in which long-lived drivers enter the system based on their expected earnings but cannot reject specific trip requests. Under their model, dynamic pricing \textit{cannot} outperform the optimal static policy in terms of throughput and revenue, but is more robust.~\citet{cachon_role_2017} argue on the other hand that surge pricing and payments are welfare increasing for all market participants when drivers decide when to work.
Similar in spirit to our work, \citet{chen_pricing_2018} consider a marketplace with forward-looking buyers and sellers who arrive sequentially and can wait for better prices in the future. They develop strategy-proof prices whose variation over time matches the participants' expected utility loss incurred by waiting.



One of the most related to our work in modeling approach, \citet{kamble_revenue_2018} considers a freelancer maximizing long-term earnings with job-length-specific prices, balancing on-job payments and utilization. In his model, a freelancer sets their own prices for a discrete number of jobs of different lengths and, with assumptions similar to our single-state model, it is optimal to set the same price per hour for all jobs. We further discuss the relationship of this work to our single-state model below.


